A Li-Yau and Aronson-B\'enilan approach for the Keller-Segel system with critical exponent

The Li-Yau and Aronson-B\'enilan estimates are fundamental differential inequalities for heat and porous-medium equations, yielding differential Harnack inequalities and sharp smoothing and decay rates. We develop analogues for the critical parabolic-elliptic Keller-Segel system on $\mathbb{R}^d$, where diffusion and aggregation act at the same scale. Our main tool is the effective pressure $v=p-u$, with $p=\log\rho$ in $d=2$ and $p=\frac{m}{m-1}\rho^{m-1}$ for $d>2$, $m=2-\frac{2}{d}$. We prove quantitative lower bounds on $\Delta v$, showing that classical pressure estimates subsist in a suitable form despite the nonlocal interaction. These estimates unify previous results and yield new regularity. For nonnegative finite-measure initial data of sufficiently small mass, assuming only a logarithmic moment in $d=2$, we construct global solutions smooth for positive times and satisfying $\|\rho_t\|_{L^\infty}\le C/t$. For finite-free-energy data, we obtain global $L^\infty$ bounds of order $1+t^{-1}$ in the subcritical and critical mass regimes. We also introduce a new characterization of the critical mass as the minimal mass $M_c^{\mathrm{sub}}(d)$ of subsolutions of the elliptic Lane-Emden equation (Liouville in $d=2$). We prove that it equals $8\pi$ in dimension $2$ and, for $d\ge3$, coincides with the Keller-Segel critical mass given by the HLS inequality, by reducing the problem to a one-dimensional optimal-control problem. Along the way we prove tools of independent interest: $L^\infty$ estimates from lower bounds on $\Delta v$, critical log-HLS/HLS estimates away from Dirac masses, Hessian bounds for Newtonian potentials, and Lipschitz and Hessian estimates for bounded porous-medium solutions with drifts on the whole space.

==> tex/commands/document.tex <==
%%% Margins
\usepackage[margin=1.0in]{geometry}

%%% Title
\makeatletter
\def\@maketitle{%
	\newpage
	\begin{center}%
		\let \footnote \thanks
		{\LARGE\bfseries \@title \par}%
		\vskip 2.5em%
			{\large
				\lineskip .5em%
				\begin{tabular}[t]{c}%
					\@author
				\end{tabular}\par}%
		\vskip 1em%
			{\large \@date}%
	\end{center}%
	\par
	\vskip 1.5em}
\makeatother

%%% Headers and Footers
\makeatletter
\let\newtitle\@title
\let\newauthor\@author
\let\newdate\@date
\makeatother
\usepackage{fancyhdr}
\pagestyle{fancy}
% Reserve enough header height without moving the text area.
\setlength{\headheight}{14pt}
\addtolength{\topmargin}{-2pt}
\lhead{}
\chead{}
\rhead{\leftmark}
\lfoot{}
\cfoot{\thepage}
\rfoot{}

\newcommand{\appendiceshead}{\rhead{\MakeUppercase{Appendices}}}
\newcommand{\referenceshead}{\rhead{\MakeUppercase{References}}}

%%% Hyperlinks
\usepackage[
	hypertexnames=false,
	pdftex,
	pdftitle={\thetitle. \authorPDF},
	pdfauthor={\authorPDF},
	pdfsubject={\subjectPDF},
	pdfkeywords={\keywordsPDF},
]{hyperref}
\hypersetup{
	colorlinks=true,
	linkcolor=black,
	citecolor=black,
	urlcolor=black,
	linktocpage
}

%%% Spacing
\usepackage{setspace}
\setstretch{1.1}

%%% Figure Placement
\usepackage{placeins}

%%% Front Matter
\newcommand{\subjectclassification}[1]{

	{\small\textbf{\textit{AMS Subject Classification --- }} #1}

}
\newcommand{\keywords}[1]{

	{\small\textbf{\textit{Keywords --- }} #1}

}

%%% Equation Numbering and Referencing
\numberwithin{equation}{section}
\usepackage[capitalise]{cleveref}

%%% Aronyms
\usepackage[nolist]{acronym}

%%%
%\usepackage{amsfonts}
%\usepackage{amsmath,amssymb,amsthm,mathrsfs,eucal,mathtools}
